Resource Allocation for Mixed RF and Hybrid RF/FSO Relaying

In this paper, we consider a mixed RF and hybrid RF/FSO system where several mobile users transmit their data over an RF link to a relay node (e.g. a small cell base station) and the relay forwards the information to a destination (e.g. a macro cell base station) over a hybrid RF/FSO backhaul link. The relay and the destination employ multiple antennas for transmission and reception over the RF links while each mobile user has a single antenna. The RF links are full-duplex with respect to the FSO link and half-duplex with respect to each other, i.e., either the user-relay RF link or the relay-destination RF link is active. For this communication setup, we derive the optimal resource allocation policy for sharing the RF bandwidth resource between the RF links. Our numerical results show the effectiveness of the proposed communication architecture and resource allocation policy, and their superiority compared to existing schemes which employ only one type of backhaul link.

==> Fig/Weather/Weather.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{018}[cl][cl]{\matlabtextA Conventional RF Relaying}%
\psfrag{019}[cl][cl]{\matlabtextA Mixed RF/FSO Relaying}%
\psfrag{020}[cl][cl]{\matlabtextA Proposed Protocol}%
\psfrag{021}[cl][cl]{\matlabtextA $d=2$ km}%
\psfrag{022}[cl][cl]{\matlabtextA $d=1$ km}%
\psfrag{023}[bc][bc]{\matlabtextA Normalized throughput, $\bar{\tau}$, (in Mbits/second)}%
\psfrag{024}[tc][tc]{\matlabtextA Weather-dependent attenuation coefficient of the FSO link, $\kappa$, $(\times 10^{-3})$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $10$}%
\psfrag{002}[ct][ct]{\matlabtextB $20$}%
\psfrag{003}[ct][ct]{\matlabtextB $30$}%
\psfrag{004}[ct][ct]{\matlabtextB $40$}%
\psfrag{005}[ct][ct]{\matlabtextB $50$}%
\psfrag{006}[ct][ct]{\matlabtextB $60$}%
\psfrag{007}[ct][ct]{\matlabtextB $70$}%
\psfrag{008}[ct][ct]{\matlabtextB $80$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextB $0$}%
\psfrag{010}[rc][rc]{\matlabtextB $100$}%
\psfrag{011}[rc][rc]{\matlabtextB $200$}%
\psfrag{012}[rc][rc]{\matlabtextB $300$}%
\psfrag{013}[rc][rc]{\matlabtextB $400$}%
\psfrag{014}[rc][rc]{\matlabtextB $500$}%
\psfrag{015}[rc][rc]{\matlabtextB $600$}%
\psfrag{016}[rc][rc]{\matlabtextB $700$}%
\psfrag{017}[rc][rc]{\matlabtextB $800$}%
%
%% </ytick>
